Search for Concepts: Discovering Visual Concepts Using Direct Optimization

Finding an unsupervised decomposition of an image into individual objects is a key step to leverage compositionality and to perform symbolic reasoning. Traditionally, this problem is solved using amortized inference, which does not generalize beyond the scope of the training data, may sometimes miss correct decompositions, and requires large amounts of training data. We propose finding a decomposition using direct, unamortized optimization, via a combination of a gradient-based optimization for differentiable object properties and global search for non-differentiable properties. We show that using direct optimization is more generalizable, misses fewer correct decompositions, and typically requires less data than methods based on amortized inference. This highlights a weakness of the current prevalent practice of using amortized inference that can potentially be improved by integrating more direct optimization elements.

==> includes/04_Applications.tex <==
\section{Applications}
\label{sec:applications}

% \input{includes/old_applications}

...


==> includes/_pseudo_code.tex <==

\begin{algorithm}
	\caption{Pseudo Code} 
    Input: I, learning rate: lr;
    
    Output:Set of parts \(\tau\) and a list of composition parameters $c_i \coloneqq (e_i, \theta_i)$ 
	\begin{algorithmic}[1]
	    \State \(Intialize~\tau
	    %, f_{residual} \leftarrow f
	    \);%(can~be~constant~or~sampled~from~a~distribution)

		\For {$iteration=1,2,\ldots$}
		
		    \(-------~Search~Phase------- \)
			\For {$layers=1,2,\ldots,N$}
            	\State \(c_n \leftarrow arg max ~ \mathcal{D}(I, \tau, J_{1,2,\ldots,n-1})\);
            	\State \(J_n \leftarrow f_t(\tau, c_n)\);
            	%\State \(f_{residual} \,\leftarrow\, Residual(f_{residual}, L_n)\);
			\EndFor
			\For {$layers=1,2,\ldots,N$}
    			\State \(c_{n} = Refine(J_{1,2,\ldots,n-1, n+1, \ldots, N})\);
            	\State \(J_n \leftarrow f_t(\tau, c_n)\);
			\EndFor
			
		    \(------- Learn~Phase------- \)
			\State \(\hat{I} = f_c(\mathcal{J})\);
% 			\State \( \omega = L(I, \hat{I})\);
			\State \( \tau \leftarrow \tau - lr * \frac{\partial L(I, \hat{I})}{\partial \tau}\);
		\EndFor
	\end{algorithmic} 
	\label{pseudo_code}
\end{algorithm}


% \begin{algorithm}
% 	\caption{$\mathcal{D}$ function}
% 	Input: $I, \mathcal{H}, J_{1,2,\ldots,n-1}$;
	
%     Output:$Corr^{\tau c \theta}~\forall~ \tau \in \{1 \twodots m\}, c \in \mathbb{R}^2, \theta \in[0,2\pi) $

%     \begin{algorithmic}[1]
%     \State \(\alpha_{a}, a = f_c(J_{1,2,\ldots,n-1})\);
%     \State \(\alpha_{b}^{e}, b^{e} = f_t(\mathcal{H}, e)~where~e \in \mathbb \tau c \theta\);
%     \State \( \hat{I} = \alpha_a a + (1-\alpha_a)\alpha_{b}^{e} b^{e}\);
%     \State \(Corr^e :=  \frac{\sum I \hat{I}}{\sqrt{\sum{I^2} \sum{\hat{I}^2}}} \);
%     \State \(We~can~parallelize~correlation~calculation~for~c \in \mathbb{R}^2\);
%     \State \(Corr := \frac{\sum I \alpha_a a + I(1-\alpha_a)\circledast \mathcal{H}}{ \sqrt{\sum I^2} \sqrt{\sum{{(\alpha_a a)}^2} + {(1-\alpha_a)}^2 \circledast {(\mathcal{H})}^2 + 2\alpha_a a (1- \alpha_a) \circledast \mathcal{H}}}\);
%     \end{algorithmic} 
% \end{algorithm}



==> includes/images/clevr_results.tex <==
\begin{figure}
\centering
  \includegraphics[width=8cm]{includes/images/media/clevr_results.pdf}%
  \caption{\label{fig:clevr_results} Clevr results showing 
  both the extracted dictionary (shapes) as well as their parameters (colors). Note that, since this analysis is in the image space, our algorithm picks up identical (3D) objects at different depths as different (image space) elements. Shadows are modelled using fuzzy element boundaries.
  }
\end{figure}


==> includes/images/dsprites_custom_results.tex <==
% \begin{figure}
% \centering
%   \includegraphics[width=8cm]{includes/images/media/dsprites_custom_results.pdf}%
%   \caption{\label{fig:dsprites_custom_results} Slot attention completely fails to do any decompostion with minor augmentation to the data distribution}
% \end{figure}


==> includes/images/tetris_results.tex <==
\begin{figure}
\centering
  \includegraphics[width=8cm]{includes/images/media/tetris_results.pdf}%
  \caption{\label{fig:tetris_results} 
  Example decomposition on the Tetris dataset, showing the learned dictionary.
  %Tetris results shows extracted dictionary elements.
  Since we do not account for reflections, mirrored elements appear as separate dictionary elements. 
  }
\end{figure}


==> includes/old_applications.tex <==
\subsection{Images}
\subsubsection{Search}
Searching the space of $c := (c_0, c_1, ..., c_N)$ is an NP hard problem. Therefore we greedyly initialize $c_i$'s one layer at a time and refine them further to get a better solution. While searching for $c_i$'s auto-regressively decreases the number of evaluated samples, searching over all possible $(e_i, \theta_i)$ is still computationally expensive. For example let us consider an input signal a 2D image of size WxHx3. Parameter $c_i$ contain where to place one of k RGBA parts from $\tau$, therefore $\theta_i$ contains the element translation parameter and $e_i$ points to the element in $\tau$. One way to search is by sampling all element id's $\hat{e_i}$ and location's $\hat{\theta_i}$, rendering all such samples using $f_t$ and selecting the best sample $(e_i, \theta_i) \leftarrow (\hat{e_i}, \hat{\theta_i})$ based the D function. This would imply that we'll render WxHxk images to computing each $c_i$.

To speed up search of $c_i$ values we use the parallel implementation of convolution operator readily available in all major deep learning frameworks. So we choose Normalized Cross Correlation(NCC) as the function D and rewrite it using convolution operations. We cast $\tau, \theta$ as $\mathcal{H} = \mathcal{H}^{rgb} * \mathcal{H}^{\alpha}$ which form filters of the convolution and we rewrite the search over $(\hat{e_i}, \hat{\theta_i})$ as a search over translations of $\mathcal{H}$.

%While this procedure does not guarantee the exact solution, it has converged to an acceptable solution mostly in our experiments. Search over

We first discuss how we perform search over possible translation in 2D for the layer without being conditioned on . Given an input image I $\in \mathcal{R}^{W*H*3}$ and part H $\in \mathcal{R}^{w*h*3}$ we need to find the (x, y) location such that we maximize $NCC(I, J_i)$
%(E.g we would like to minimize mean squared error or maximize the correlation).
%In this work we use Normalized Cross Correlation(NCC) as the energy function D, we explain why choose NCC later in this section. 
\begin{equation}
    D(x, y) = \frac{\sum I \hat{I}}{\sqrt{\sum{I^2} \sum{\hat{I}^2}}} \\
\label{eq:NCC}
\end{equation}

where
\begin{equation}
     \hat{I}(x+n, y+m) =  
    \left\{\begin{array}{ll}
        H(n,m) & \text{if}\ \ 0<n<w \\
               & \ \ \ \ 0<m<h, \\
        0 & \text{if}\ \ n>w \\ 
          & \ \ \ \ m>h,
        \end{array}\right.
\label{eq:translation}
\end{equation}
we can rewrite the eq\ref{eq:NCC}, \ref{eq:translation} as
\begin{equation}
    D = \frac{I \circledast H}{\sqrt{\sum{I^2} (\mathbf{1} \circledast {H^2})}} \\
\label{eq:NCC_single_rewrite}
\end{equation}
Where $\mathbf{1}$ $\in \mathcal{R}^{W*H*3}$ and contains value 1 and $\circledast$ is the convolution operator. Note how choosing NCC over mean squared error help's us take advantage of parallel implementations of $\circledast$ function. 

Given D output of eq. \ref{eq:NCC_single_rewrite} $J_i = f_t(\tau, c_i)$ where $c_i = \argmax_{(x,y)}(D)$ one can think of this as a voting between different samples of $c_i$.
Notice that the D function in eq. \ref{eq:NCC_single_rewrite} is not conditioned on $J_{0,1, ..., i-1}$ so it can only be used to initalize $c_0$. How $J_{0,1, ..., i-1}$ effect searching $c_i$ values depends on the composition function of choice. 
%The context is based on the composition function. 
Let us consider the traditional compositional function for 2D images eq. \ref{eq:traditional_compositing} 

\begin{equation}
    f_c(J_{0, 1, ..., i}, bg) = \sum_{i=1}^{n} [ J^{rgb}_i * J^{\alpha}_{i} \prod_{j=1}^{n-1} (1-J^{\alpha}_{j})] + bg * \prod_{i=1}^{n} (1-J^{\alpha}_{i})
    \label{eq:traditional_compositing}
\end{equation}

for the sake of simplicity: 
\begin{equation}
  \begin{array}{l}
    J_a^{rgb}, J_a^{\alpha}=f_c(J_{0, 1, ..., i-1}, 0) \\
    J_b^{rgb}, J_b^{\alpha}=f_c(J_{i}, 0) \\
    J_c^{rgb}, J_c^{\alpha}=f_c(J_{i+1, i+2, ..., n}, bg)
    \label{eq:a_rewrite}
    \end{array}
\end{equation}
%then we can rewrite eq. \ref{eq:translation} as
% \begin{equation}
%     f_c(J_{0, 1, ..., i-1}, 0) J_a^{rgb}, J_a^{\alpha}=
%     \label{eq:a_rewrite}
% \end{equation}


When we rewrite eq. \ref{eq:traditional_compositing} using eq. \ref{eq:a_rewrite} and replace in \ref{eq:NCC} and rewrite it using $\circledast$ as 
\begin{equation}
D = \frac{\sum I J_a^{\alpha} J_a^{rgb} + I(1-J_a^{\alpha})\circledast \mathcal{H}}{ \sqrt{\sum I^2} \sqrt{\sum{{(J_a^{\alpha} J_a^{rgb})}^2} + {(1-J_a^{\alpha})}^2 \circledast {(\mathcal{H})}^2 + 2J_a^{\alpha} J_a^{rgb} (1- J_a^{\alpha}) \circledast \mathcal{H}}}
    \label{eq:ours_2d_search}
\end{equation}

\begin{equation}
    num = \sum I J_a^{\alpha} J_a^{rgb} + I(1-J_a^{\alpha})\circledast \mathcal{H} + \sum I(1-J_a^{\alpha}) J_c^{rgb} - I(1-J_a^{\alpha})J_c^{rgb} \circledast J_b^{\alpha}
\end{equation}
\begin{equation}
    denom1 = \sum (J_a^{\alpha} J_a^{rgb})^2 + (1-J_a^{\alpha})^2 \circledast (J_a^{\alpha} J_a^{rgb} )^2
\end{equation}
\begin{equation}
    denom2 = \sum ((1-J_a^{\alpha}) J_c^{rgb})^2 + ((1-J_a^{\alpha}) J_c^{rgb})^2 \circledast (J_a^{\alpha})^2 - 2*((1-J_a^{\alpha}) J_c^{rgb})^2 \circledast J_a^{\alpha}
\end{equation}
\begin{equation}
    denom3 = 2 * J_a^{\alpha} J_a^{rgb}(1-J_a^{\alpha}) \circledast \mathcal{H} 
\end{equation}
\begin{equation}
    denom4 = \sum J_a^{\alpha} J_a^{rgb}(1-J_a^{\alpha})J_c^{rgb} - J_a^{\alpha} J_a^{rgb}(1-J_a^{\alpha})J_c^{rgb} \circledast \mathcal{H}^{\alpha}
\end{equation}
\begin{equation}
    denom5 = \sum 2(1-J_a^{\alpha})^2 J_c^{rgb} \circledast \mathcal{H}^{\alpha} - 2(1-J_a^{\alpha})^2 J_c^{rgb} \circledast \mathcal{H} \mathcal{H}^{\alpha}
\end{equation}




\begin{equation}
D = \frac{num}
{ \sqrt{\sum I^2} \sqrt{denom1 + denom2 + denom3 + denom4 + denom5}}
    \label{eq:ours_2d_search}
\end{equation}


\input{includes/_pseudo_code}
\subsubsection{Refine}

\ref{eq:ours_2d_search} Tries to explain the input I in a greedy way so it tries to select the largest shapes that partially explain the input image I first. There we need to perform a refinement step to explain the input image more accurately. 
We use two variant of refinement in our experiments. Each variant improves the robustness of the search procedure in different ways. The z buffer sorting refinement try to improve the occlusion ordering of the greedy initialization. The redo local search refinement tries to improvement upon the initial $c_i$ prediction. While using both the refinement steps is useful for any dataset we use them selectively based on the dataset. 

Z buffer sorting: In the z buffer sorting step we first move each layer to the front of the z buffer. After moving the layer we compute the MSE between the new augmented $c_0, c_1, ..., c_n$ and the input signal. If retain the augmentation if augmented z buffer has a lower mse value than the old z buffer. 

Conditional Redo search: In the conditional redo search step we redo the $c_i$ search in-place conditioned on $c_0, c_1, ..., c_n$. \preddy{note to self: see if I can fine a dsprites example here}. In our experiments we have noticed that this step helps when there is ambiguity between the parts for example when there are no color ques.   
%We have tried two variant of refinement one more computationally expensive than other. In our experiment both the algorithms have similar performance. We present the computationally expensive version of refinement in the supplementary. In the supplementary we also discuss how the expensive version can be more robust to certain arrangement of objects. 
\input{includes/images/refinementWandWO}

\subsection{Clones}
Convergence of $\tau$ depends on its initialization. \preddy{Give an example here.}
We clone $\tau_i$ based on two metrics, one to measure the local similarity between $\tau_i$ and the input signal and number of times $\tau_i$ is used. We use masked NCC \ref{eq:NCC_masked} as the local similarity metric. We clone $\gamma_i > \rho \sum \gamma_i$ and if local similarity metric is greater than $\lambda$ where $\lambda$ is a hyper-parameter set to 0.95. Where $\gamma_i$ is the number of times part i is used. 

\begin{equation}
    D(x, y) = \frac{\sum M I * \hat{I}M}{\sqrt{\sum{I^2} \sum{\hat{I}^2}}} \\
\label{eq:NCC_masked}
\end{equation}

We remove $\tau_i$ only based on usage. Let number of times a part $\tau_i$ used be $\gamma_i$. We $\tau_i$ if  $\gamma_i < \rho \sum \gamma_i$ where $\rho$ is a hyperparameter, we use 0.25 as $\rho$ in our experiments.
\input{includes/images/cloningWandWO}
\input{includes/images/cloneGraph}

\subsection{Training}
We use the proposed parameters from the search phase and create and composite image $\hat{I}$. We compare $\hat{I}$ with the input image I and optimize $\mathcal{H}$ using stochastic gradient descent(SGD) algorithm. In practice we use AdaDelta variant of gradient descent algorithm. However in the supplementary we show the convergence of our method using different variants of SGD. We show that our method converges with all the SGD variant with different number of steps showing the robustness. 

==> includes/old_method.tex <==
\subsection{Search}
Given an input composited signal I, in the search phase of the algorithm our aim to find the parameters $c_i$ for each layer $J_i$. 
%This involves a search which include compositional reuse parameters like translation, rotation e.t.c and their respective ids in $\tau$. 
Parameters of $c$ that form layers $\mathcal{J}$ are selected to maximize a function $D$. We maximize wrt $D$ since $D$ function metric is higher if input and estimate are similar to each other. We explain our choice of $D$ further in the next section. Brute force search operation over all possible part references $e$ and how they are used $\theta$ is computationally expensive. The search space grows exponentially with number of entries of $\tau$, the dimensions of $\theta$ and number of layers $N$. Our first observation is to explain the input signal I we can perform the search for each layer's parameter $c_i$ in an auto-regressive manner conditioned over ($c_0, c_1, ..., c_{i-1}$). During the auto-regressive search we choose each $c_i$ to maximize $D$ as much as possible. This greedy approach might not result in the perfect solution, therefore we use the first estimated $c_i$'s  as an initialization and further refine each $c_i$ conditioned on the others ($c_0, c_1, ..., c_{i-1}, c_{i+1}, ..., c_n$). This greedy initialization along with the refinement gives us $c$ values which we'll use in the learning phase.

\subsection{Learn}
Given $c$ in the learning we try to optimize $\tau$. Using $c$ we first create or render the individual layers $J_i$ using the $f_t$ function. This function creates a single layer $J_i$ using the compositional parameters $c_i$ and the parts $\tau_i$. 
Once the individual layers are created we use the compositing function $f_c$ to combine all the layers into a single signal $\hat{I}$.
We compute the different between estimated single $\hat{I}$ and the input I using a loss function $L$.
We optimize $\tau$ to either minimize $L$ if $L \propto 1/D$ or maximize $L$ if $Loss \propto D$. 
In our experiment we use gradient descent for training $\tau$.  


Depending on the initialization of $\tau$ gradient descent sometimes get stuck in local minima's between the mean value depending on how close each part variables are to each other and the data. Therefore we employ a heuristic cloning strategy that help each $\tau$ value specialize to a specific part.

==> includes/tables/notations_table.tex <==
\begin{table}[b!]
\caption{Notations used in this paper.}
\label{tab:notations}
\begin{tabular}{r|p{0.6\columnwidth}}
symbol                      & description                   \\
\hline \hline
$\mathcal{I}$               & Image dataset.                         \\ 
$I$                         & Input RGBA image.                         \\
$\tilde{I}$                 & Reconstructed RGBA image.                         \\
$\mathcal{V}$                         & Dictionary of visual concepts.          \\
$V_j \in \mathcal{V}$                 & Visual concept $j$ of the dictionary. \\
$L_i$                       & Layer $i$ of the image $I$.                         \\ 
$\hat{L}_i$                 & Layer with zeroed transl. params.                         \\ 
$l_\mathcal{V}(\theta)$               & Parametric layer generator.                         \\ 
$\theta_i \coloneqq (\tau_i, \phi_i)$                  & Parameters of layer $L_i$.                             \\
$\tau_i$                    & Index of the visual concept in $L_i$.            \\
$\phi_i$                    & Transform. params. of layer $L_i$.            \\
$T(\tau, \phi)$         & Visual concept transform. function. \\ 
$h$                         & Image composition function.            \\
\end{tabular}
\end{table}
